MoDiTalker: Motion-Disentangled Diffusion Model for High-Fidelity Talking Head Generation

Conventional GAN-based models for talking head generation often suffer from limited quality and unstable training. Recent approaches based on diffusion models aimed to address these limitations and improve fidelity. However, they still face challenges, including extensive sampling times and difficulties in maintaining temporal consistency due to the high stochasticity of diffusion models. To overcome these challenges, we propose a novel motion-disentangled diffusion model for high-quality talking head generation, dubbed MoDiTalker. We introduce the two modules: audio-to-motion (AToM), designed to generate a synchronized lip motion from audio, and motion-to-video (MToV), designed to produce high-quality head video following the generated motion. AToM excels in capturing subtle lip movements by leveraging an audio attention mechanism. In addition, MToV enhances temporal consistency by leveraging an efficient tri-plane representation. Our experiments conducted on standard benchmarks demonstrate that our model achieves superior performance compared to existing models. We also provide comprehensive ablation studies and user study results.

==> assets/figures/qual_teaser.tex <==
\begin{center}
    \centering
    \captionsetup{type=figure}
    \includegraphics[width=1\textwidth]{assets/figures/1_th_teaser.png}
    \vspace{-15pt}
    \captionof{figure}{We present the \textbf{Mo}tion-\textbf{Di}sentangled diffusion model for high-fidelity \textbf{Talk}ing head gen\textbf{er}ation, dubbed \textbf{MoDiTalker}. This framework generates high-quality talking head videos through a two-stage, motion-disentangled diffusion models.}
    \label{fig:teaser}
\end{center}%

==> assets/tables/abl_atom.tex <==
\begin{wraptable}{r}{3cm}
    \centering
    \resizebox{1 \linewidth}{!}{
    \begin{tabular}{c|l|ccccc}\toprule
    
        & Method & LMD $\downarrow$  & Lip-sync $\uparrow$   \\\midrule 
        
        & GeneFace~\cite{ye2023geneface} &{137.52} & {0.339}\\ \midrule
        
        (\textbf{I}) & Baseline  & {159.47} & {0.316}\\ 
        
        (\textbf{II}) & (\textbf{I}) + Residual. &{143.73} &{0.386} \\
        
        (\textbf{III}) & (\textbf{II}) + $F_L$ & {128.65} & {0.385}\\ \hlrow
        
        (\textbf{IV}) & (\textbf{III}) + Disen. Att. (\textbf{Ours}) &\textbf{123.55} &\textbf{0.389} 
        
        \\ \bottomrule
    \end{tabular}}
    \caption{\textbf{Component analysis on AToM.}}
    \label{tab:atom_ablation}
\end{wraptable}


% \begin{table}[t]
%     \centering
%     \resizebox{1
%     \columnwidth}{!}{
%     \begin{tabular}{c|l|ccc}
%         \toprule
%         & Component & $I_\mathrm{DINO}$ $\uparrow$ & $I_\mathrm{CLIP}$ $\uparrow$ &  $T_\mathrm{CLIP}$ $\uparrow$ \\
%         \midrule
%         (I) & Baseline (DreamBooth~\cite{ruiz2023dreambooth}) &0.638 &0.808 & 0.237 \\
%         \midrule
%         (II) & (I) + Key-Value Replacement (MasaCtrl~\cite{cao2023masactrl}) & 0.728 & 0.854 & 0.201 \\
%         \midrule
%         (III) & (I) + Semantic Matching &0.683&0.830&0.201 \\
%         (IV) & (III) + Semantic-Consistent Mask (AMA)
%           &0.676&0.818&0.232\\
%         (V) & (IV) + Semantic Matching Guid. (Ours) &0.680 &0.821 & 0.231\\
%         \bottomrule
%     \end{tabular}
%     }
%     \vspace{-5pt}
%     \caption{\textbf{Component analysis.} For this analysis, we used DreamBooth~\cite{ruiz2023dreambooth} for the baseline.}
%     \vspace{-10pt}
%     \label{quan:comp_analysis}
%     \end{table}

==> assets/tables/abl_atom_new_table.tex <==
\begin{table}[t]
    \centering
    \resizebox{1
    \columnwidth}{!}{
    \begin{tabular}{c|l|ccc}
        \toprule
        & Component & $I_\mathrm{DINO}$ $\uparrow$ & $I_\mathrm{CLIP}$ $\uparrow$ &  $T_\mathrm{CLIP}$ $\uparrow$ \\
        \midrule
        (I) & Baseline (DreamBooth~\cite{ruiz2023dreambooth}) &0.638 &0.808 & 0.237 \\
        \midrule
        (II) & (I) + Key-Value Replacement (MasaCtrl~\cite{cao2023masactrl}) & 0.728 & 0.854 & 0.201 \\
        \midrule
        (III) & (I) + Semantic Matching &0.683&0.830&0.201 \\
        (IV) & (III) + Semantic-Consistent Mask (AMA)
          &0.676&0.818&0.232\\
        (V) & (IV) + Semantic Matching Guid. (Ours) &0.680 &0.821 & 0.231\\
        \bottomrule
    \end{tabular}
    }
    \vspace{-5pt}
    \caption{\textbf{Component analysis.} For this analysis, we used DreamBooth~\cite{ruiz2023dreambooth} for the baseline.}
    \vspace{-10pt}
    \label{quan:comp_analysis}
    \end{table}

==> assets/tables/abl_computation.tex <==

% \begin{wraptable}{r}{6cm}
% \begin{center}
% \resizebox{6cm}{!}{%{
% \begin{tabular}{lcccc}
%     \toprule
%         Method 
%         & DiffTalk~\cite{shen2023difftalk} 
%         & DiffusedHead~\cite{stypułkowski2023diffused} 
%         & \textbf{MoDiTalker}
%         \\\midrule 
%          inference time     
%          \quad &{1,003s}  
%          \quad & {716s} 
%          \quad & {23s}
%          \\ \bottomrule
%     \end{tabular}%
%     }
% \end{center}
%     \vspace{2pt}
%     \caption{Comparison the time spent on generating a 25fps, 5-second video using diffusion-based methods}
%     \label{tab:training_inference_efficiency}
% \end{wraptable}

\begin{wraptable}{r}{4.5cm}
\begin{center}
\resizebox{4.5cm}{!}{%{
\begin{tabular}{lc}
    \toprule
        Method & Inference time

        \\\midrule
         DiffTalk~\cite{shen2023difftalk} & {1,003} \\ 
        DiffusedHead~\cite{stypułkowski2023diffused} 
        & {716} 

        \\
        \textbf{Ours}
        & {23}

         \\ \bottomrule
    \end{tabular}%
    }
\end{center}
    \vspace{-5pt}
    \caption{Comparison the time spent on generating a 25fps, 5-second video using diffusion-based methods}
    \label{tab:training_inference_efficiency}
\end{wraptable}

==> assets/tables/main.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l cc cc ccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Lip Synchronization} & \multicolumn{2}{c}{Learned Head Motion}  & \multicolumn{3}{c}{Video Quality} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-8}
& LSE-C$\uparrow$ & LSE-D$\downarrow$ & Diversity$\uparrow$ & Beat Align$\uparrow$ & FID$\downarrow$ & CPBD$\uparrow$ & CSIM$\uparrow$ \\
\hline % 0.271 &
Real Video & 8.211 & 6.982 & 0.259 & 0.271 & 0.000 & 0.428 &1.000 \\
\rowcolor{lightgray!30} Wav2Lip*~\cite{wav2lip} & 10.221 &5.535  &N./A. & N./A. &21.725 &0.368 &0.849\\
\rowcolor{lightgray!30} PC-AVS**~\cite{pcavs} &9.053 &6.355  & N./A. & N./A. &69.127 &0.206 &0.683\\
MakeItTalk~\cite{zhou2020makelttalk} &5.110 &10.059  &0.257 &0.268 &28.243 &0.283 &0.838\\
Audio2Head~\cite{wang2021audio2head} &7.357 &7.535   &0.181 &0.267 &24.392 &0.281 &0.823\\
Wang~\etal~\cite{wang2021one} &4.932 &10.055 &0.226 &0.268 &22.432 &0.295 &0.811 \\
% PIRenderer~\cite{ren2021pirenderer} & automatic \\
Ours & 7.290 &7.772 & \textbf{0.278} & \textbf{0.293} & \textbf{22.057} & \textbf{0.335} & \textbf{0.843} \\
\bottomrule
\end{tabular}
\vspace{-1em}
\caption{
Comparison with the state-of-the-art method on HDTF dataset. We evaluate Wav2Lip~\cite{wav2lip} and PC-AVS~\cite{pcavs} in the one-shot settings. Wav2Lip* achieves the best video quality since it only animates the lip region while other regions are the same as the original frame. PC-AVS** is evaluated using the fixed reference pose and fails in some samples.
}
\vspace{-0.05in}
\label{tab:compare}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l c c c c c c }\toprule
         &\multicolumn{2}{c}{CelebA-HQ~\cite{liu2015deep}}
         &\multicolumn{2}{c}{AnimalFaces-10~\cite{liu2019few}}
         &\multicolumn{2}{c}{Food-10~\cite{bossard2014food}}\\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        Method &mFID $\downarrow$  &D\&C $\uparrow$ &mFID $\downarrow$ &D\&C $\uparrow$ &mFID $\downarrow$ &D\&C $\uparrow$ \\\midrule 
        StarGAN2~\cite{choi2020starganv2} (sup.) &32.16 &1.22 / \textbf{0.44} &\textbf{33.67} &\textbf{1.54} / \textbf{0.91} &65.03 &1.09 / 0.76 \\
        Smoothing~\cite{liu2021smoothing} (sup.) &35.93 &\textbf{1.25} / 0.43 &38.93 &0.97 / 0.75 &61.13 &0.96 / 0.68 \\ 
        TUNIT~\cite{baek2021rethinking} (unsup.) &61.29 &0.24 / 0.13 &47.70 &1.04 / 0.81 &52.20 &1.08 / \textbf{0.88}  \\
        Kim \textit{et al}.~\cite{kim2022style} (unsup.) &41.33 &0.60 / 0.24 &36.83 & 1.06 / 0.82 &49.34 &1.06 / 0.80  \\ \rowcolor{red!7} 
        LANIT &\textbf{27.96} &0.91 / 0.34 & 34.11 &1.46 / 0.89 &\textbf{48.08} &\textbf{1.24} / 0.86 \\\bottomrule
    \end{tabular}
    \vspace{-1mm}
    \caption{\textbf{Quantitative comparison on CelebA-HQ~\cite{liu2015deep}, Animal Faces-10~\cite{liu2019few} and Food-10~\cite{bossard2014food}} The configurations of StarGAN2 and Smoothing use ground-truth domain labels while TUNIT and Kim \textit{et al}. use pseudo-labels generated from each image. Our LANIT uses only textual domain descriptions.}
    \label{tab:quan_table}
    % \vspace{-10pt}
\end{table*}
